Quantifying an Interference-Assisted Signal Strength Breathing Surveillance Attack

A malicious attacker could, by taking control of internet-of-things devices, use them to capture received signal strength (RSS) measurements and perform surveillance on a person's vital signs, activities, audio in their environment, and other RF sensing capabilities. This paper considers an attacker who looks for periodic changes in the RSS in order to surveil a person's breathing rate. The challenge to the attacker is that a person's breathing causes a low amplitude change in RSS, and RSS is typically quantized with a significantly larger step size. This paper contributes a lower bound on an attacker's breathing monitoring performance as a function of the RSS step size and sampling frequency so that a designer can understand their relationship. Our bound considers the little-known and counter-intuitive fact that an adversary can improve their sinusoidal parameter estimates by making some devices transmit to add interference power into the RSS measurements. We demonstrate this capability experimentally. As we show, for typical transceivers, the RSS surveillance attack can monitor RSS with remarkable accuracy. New mitigation strategies will be required to prevent RSS surveillance attacks.

==> problem.tex <==

\section{RSS Model for Breathing}
\label{sec:model}

To analyze the theoretical limits on breathing eavesdropping, we model the breathing-induced RSS signal. Past work has demonstrated the validity of modelling of breathing induced RSS as a sinusoid with DC offset \cite{patwari2014monitoring}. Therefore, we assume that a person's vital sign changes the measured signal as an additive sinusoidal component.  Although generally an eavesdropper may take burst RSS measurements, we assume a scalar time-dependant signal for simplicity.  We use $B$ to denote the signal when breathing is absent, and $v(k)$ to denote the noise in sample $k$, which is assumed to be zero-mean white Gaussian noise with variance $\sigma^2$.  Therefore, the sampled signal is given as
\begin{equation} \label{eqn:model}
    x[k] = A\cos{(\omega T_s k+\phi)}+B + v[k],  \qquad k \in \mathbb{Z}
\end{equation}
where $T_s$ is the sampling period and the breathing signal has unknown amplitude $A$, DC offset $B$, frequency $\omega$, and the initial phase $\phi$. The unknown parameter vector is defined as $\bm{\theta} = [A, B,\omega,\phi]^T$.  Our goal is, in particular, to estimate $A$ and $\omega$, which are of medical interest.

The signal $x(k)$ goes through one-bit quantization. The output of the quantization is in the set $\{-1,1\}$ and given by
\begin{eqnarray} \label{eqn:quantization}
y[k] &=& {\rm sign}\left(x[k]-\zeta\right)
\end{eqnarray}

where $\zeta$ is the threshold for quantization and the sign function ${\rm sign}(\cdot)$ is defined as ${\rm sign}(x)=1$ for $x\geq0$ and ${\rm sign}(x)=-1$ for $x < 0 $. Without loss of generality, we assume $\zeta=0$.  We define ${\bm y} = \left[y[0], \ldots, y[N-1]\right]^T$ to be our measurement vector.

